Constant Approximation for Private Interdependent Valuations

The celebrated model of auctions with interdependent valuations, introduced by Milgrom and Weber in 1982, has been studied almost exclusively under private signals $s_1, \ldots, s_n$ of the $n$ bidders and public valuation functions $v_i(s_1, \ldots, s_n)$. Recent work in TCS has shown that this setting admits a constant approximation to the optimal social welfare if the valuations satisfy a natural property called submodularity over signals (SOS). More recently, Eden et al. (2022) have extended the analysis of interdependent valuations to include settings with private signals and private valuations, and established $O(\log^2 n)$-approximation for SOS valuations. In this paper we show that this setting admits a constant factor approximation, settling the open question raised by Eden et al. (2022).

==> figures/valuations.tex <==
\def\scale{.6}
\begin{tikzpicture}[very thick,scale=\scale]
\draw[densely dotted, name path=binary] (-9,0) -- (12,0);
\draw[densely dotted, name path=monotone] (0,-5.8) -- (0,7);
\node at (10,.5) {\footnotesize $\{0,1\}$ signals};
\node at (10,-.5) {\footnotesize $[0,1]$ signals};
\node at (2,6.5) {\footnotesize\begin{minipage}{2cm}\raggedright
monotone\\valuations\end{minipage}};
\node at (-2,6.5) {\footnotesize\begin{minipage}{2cm}\raggedleft
non-monotone\\valuations\end{minipage}};
\node at (10,3) {\footnotesize 2-\selfbounding};
\node at (10,2) {\footnotesize 1-\selfbounding};
\draw[dashed] (8,2.5) rectangle (12,1.5);
\draw (7.8,3.5) rectangle (12.2,1.3);
\begin{scope}
    \node at (10,-5.1) {\footnotesize OSos};
    \begin{scope}[xshift=10cm, yshift=-5.1cm, scale=.3]
        \draw (-4,-1) -- (-2,1) -- (2,1) -- (4,-1) -- cycle;
    \end{scope}
    \draw (-4,-1) -- (-2,1) -- (2,1) -- (4,-1) -- cycle;
\end{scope}
\begin{scope}
    \node[rotate=-90] at (9,-3.5) {\footnotesize XSos};
    \begin{scope}[xshift=9cm, yshift=-3.5cm, scale=.3]
        \draw (-1,-4) -- (1,-2) -- (1,2) -- (-1,4) -- cycle;
    \end{scope}
    \draw (-1,-4) -- (1,-2) -- (1,2) -- (-1,4) -- cycle;
\end{scope}
\draw[dashed] (-5,-5) rectangle (5,5);
\draw (-7,-5.5) rectangle (7,5.5);
\begin{scope}[blue!50!black]
    \node at (10.5,-4) {\footnotesize Sos};
    \begin{scope}[xshift=10.7cm, yshift=-4cm, scale=.17]
        \draw (-6,-3) -- (2.375,-3) -- (4.25,-1.125) -- (4.25,1.125) -- (2.375,3) -- (-6,3) -- cycle;
    \end{scope}
    \draw (-6,-3) -- (2.375,-3) -- (4.25,-1.125) -- (4.25,1.125) -- (2.375,3) -- (-6,3) -- cycle;
    \node at (10,4.5) {\footnotesize Submodular set function};
    \fill[opacity=0.1] (7.5,4) rectangle (12.5,5);
    \begin{scope}
        \clip (-10,0) rectangle (10,5);
        \fill[opacity=0.1] (-6,-3) -- (2.375,-3) -- (4.25,-1.125) -- (4.25,1.125) -- (2.375,3) -- (-6,3) -- cycle;
    \end{scope}
    \begin{scope}
        \clip (0,-5) rectangle (10,5);
        \draw[pattern=north east lines,opacity=0.3] (-6,-3) -- (2.375,-3) -- (4.25,-1.125) -- (4.25,1.125) -- (2.375,3) -- (-6,3) -- cycle;
    \end{scope}
    %\fill[opacity=0.1, intersection segments={of=binary and Sos}];
\end{scope}
\begin{scope}[red!50!black]
    \node at (10.5,-2.5) {\footnotesize XOSos};
    \begin{scope}[xshift=10.5cm, yshift=-2.5cm, scale=.17]
        \draw (-1.25,4.5) -- (1.25,4.5) -- (4.5,1.25) -- (4.5,-1.25) -- (1.25,-4.5) -- (-1.25,-4.5) -- (-4.5,-1.25) -- (-4.5,1.25) -- (-1.25,4.5);
    \end{scope}
    \draw (-1.25,4.5) -- (1.25,4.5) -- (4.5,1.25) -- (4.5,-1.25) -- (1.25,-4.5) -- (-1.25,-4.5) -- (-4.5,-1.25) -- (-4.5,1.25) -- (-1.25,4.5);
    \node at (10,5.7) {\footnotesize XOS set function};
    \fill[opacity=0.1] (7.5,5.2) rectangle (12.5,6.2);
    {
        \clip (0,0) rectangle (10,5);
        \fill[opacity=0.1] (-1.25,4.5) -- (1.25,4.5) -- (4.5,1.25) -- (4.5,-1.25) -- (1.25,-4.5) -- (-1.25,-4.5) -- (-4.5,-1.25) -- (-4.5,1.25) -- (-1.25,4.5);
    }
\end{scope}
\begin{scope}[green!50!black]
    {
        \small
        \node at (-8,-6.2) {$x\cdot(1-y)$};
        \node at (-4.5,-6.2) {$x+1-y$};
        \node at (-1,-6.2) {$\max(x, 1-y)$};
        \node at (6.6,-6.2) {$x\cdot y$};
        \node at (4.8,-6.2) {$x+y$};
        \node at (2.4,-6.2) {$\max(x,y)$};
    }
    \fill (-5.5, -0.5) circle (.1cm);
    \fill (-.7, -3.4) circle (.1cm);
    \fill (6.6, -0.5) circle (.1cm);
    \fill (.5, -1.5) circle (.1cm);
    \fill (1.5, -.5) circle (.1cm);
    \fill (-1.5, -.5) circle (.1cm);
    \begin{scope}[->,>=stealth, rounded corners=1.2*\scale cm]
        \draw (-8,-5.8) -- (-8,-.5) -- (-5.5,-.5);
        \draw (-4.5,-5.8) -- (-4.5,-.5) -- (-1.5,-.5);
        \draw (-.7,-5.8) -- (-.7,-3.4);
        \draw (6.6,-5.8) -- (6.6,-.5);
        \draw (2.4,-5.8) -- (2.4,-1.5) -- (.5,-1.5);
        \draw (4.8,-5.8) -- (4.8,-.5) -- (1.5,-.5);
    \end{scope}
\end{scope}
\end{tikzpicture}
